Twinner: Shining Light on Digital Twins in a Few Snaps

We present the first large reconstruction model, Twinner, capable of recovering a scene's illumination as well as an object's geometry and material properties from only a few posed images. Twinner is based on the Large Reconstruction Model and innovates in three key ways: 1) We introduce a memory-efficient voxel-grid transformer whose memory scales only quadratically with the size of the voxel grid. 2) To deal with scarcity of high-quality ground-truth PBR-shaded models, we introduce a large fully-synthetic dataset of procedurally-generated PBR-textured objects lit with varied illumination. 3) To narrow the synthetic-to-real gap, we finetune the model on real life datasets by means of a differentiable physically-based shading model, eschewing the need for ground-truth illumination or material properties which are challenging to obtain in real life. We demonstrate the efficacy of our model on the real life StanfordORB benchmark where, given few input views, we achieve reconstruction quality significantly superior to existing feedforward reconstruction networks, and comparable to significantly slower per-scene optimization methods.

==> sec/1_intro_old.tex <==
\section{Introduction [OLD]}
\label{sec:intro}

% Contributions:
% \begin{itemize} 
% \item Fully-differentiable PBR renderer integrating predicted environment light on the surface of meshes textured with PBR materials
% \item Large-data training on real-life (co3dv2) and synthetic (envmap-zeroverse) data
% \item SOTA feedforward environment map predictor
% \item Tricolumn representation
% \end{itemize}

% story:
% - digital twins are important since we can use them for many things
% - NeRF or 3DGS have shown strong progress in this area, however the assets generated by these methods have baked light
% - As such, methods such as NVDiffRec, NeRF, NeRFactor decompose to PBR, but are ill-posed
% - Recently, AssetGen has shown that feedforward PBR reconstruction is possible, but requires a large dataset of PBR-annotated assets. Existing datasets are bad.
% - To deal with the latter, we propose a novel feedforward predictor of PBR-textured assets designed to handle real-life input images. 
% We also introduce a large dataset of synthetic PBR-textured assets with environment maps to supercharge learning of environment maps. Finally, we improve the 3D representation with a novel "Tricolumn"-based architecture that scales only quadratically with the size of the voxel grid while a standard patch-based transformer would scale cubically.
% - We tackle the problem with two tricks:
% - 1) Fully differentiable feedforward env map predictor allowing to train on real life data
% - 2) Large dataset of synthetic PBR-textured assets with environment maps to supercharge learning of envmaps
% - Finally, we also improve the 3D representation with a novel "Tricolumn"-based architecture that scales only quadraticaly with the size of the voxel grid while a stadard patch-based transformer would scale cubically.
% - We demonstrate the efficacy of our model on the real-life StanfordORB benchmark where, given few input views, we achieve performance significantly superior to existing feedforward methods, and performance comparable to significantly slower scene optimization methods.

Digital twin creation, or the task of converting real-world objects into 3D assets, is a crucial one with many applications in virtual, augmented reality, and general 3D content creation.
In the last few years, strides in implicit shape reconstructors such as NeRF \cite{mildenhall20nerf:}, 3D Gaussian Splatting \cite{kerbl233d-gaussian}, or their feedforward versions \cite{henzler2021unsupervised,yu21pixelnerf:,tang24lgm:,xu24grm:} significantly increased the popularity of digital twinning.
However, traditional implicit shape methods have a significant drawback: Since the scene's texture is modelled via radiance, or the color of the light emitted from the scene's surface to all directions, such assets look out-of-place in other scenes with different lighting conditions.

Hence, methods such as NVDiffRec \cite{munkberg2022extracting}, NeRD \cite{boss2021nerd}, NeRFactor \cite{zhang2021nerfactor}, replace radiance with a decomposition of the scene texture to Physically-based Rendering texture planes (albedo, roughness, metallicity).
Combined with an environment light, which is also optimized, the scene is rendered with a differentiabe PBR shader to evaluate a photometric error that supervises the fitting process. 
Unfortunately, the latter problem is massively overparametrized and, hence, ill-posed making the optimization notoriously hard.

Recently, AssetGen \cite{siddiqui2024meta} successfully tackled PBR decomposition by means of a feedforward architecture. 
Here, MetalLRM, an enhancement of the LightplaneLRM \cite{cao2024lightplane} reconstructor, directly predicts PBR-textured assets from input object images without relying on the ill-posed optimization. 
However, the model requires supervision with a large dataset of PBR-annotated assets. 
Unfortunately, current 3D asset datasets, such as Objaverse \cite{deitke23objaverse:}, contain PBR-textures of insufficient quality. 
Moreover, MetalLRM, due to being tailored for 3D asset generation, performs poorly on digital twinning of real-life objects.

We thus propose a novel feedforward predictor of PBR-textured assets dubbed \themethod designed to significantly improve the quality of PBR textures predicted from real-life input images.
Following MetalLRM, \themethod is a large transformer-based model which predicts a PBR-textured opacity field.
Importantly, \themethod deals with the scarcity of high-quality ground-truth PBR-shaded models by means of two key innovations.

First, we significantly increase the amount of training data by exploiting real object-centric captures from CO3Dv2
% by introducing a novel fully-differentiable PBR renderer.
Since real scenes lack ground-truth PBR annotations, we supervise the PBR prediction indirectly.
More specifically, we endow \themethod with an additional prediction head that estimates the scene's environment light.
During training, the scene is rendered with a fully-differentiable PBR shader that calculates the reflections of the predicted environment light from the surface of the predicted PBR asset.
The latter then admits PBR supervision via photometric losses between the renders and the corresponding real ground-truth images.

Second, we further enlarge the training set with a large fully-synthetic dataset of procedurally generated PBR-textured objects lit with a known environment light.
The latter not only gives more supervisory signal for the PBR predictor, but the ground-truth environment map annotations also allow to directly supervise \themethod's environment-light prediction branch.

Finally, we improve general reconstruction quality by replacing the tripane 3D representation of MetalLRM with a more expressive voxel grid of latent features.
Here, a key challenge is the high memory complexity of MetalLRM's transformer which scales cubically with the size of the voxel grid.
To this end, \themethod introduces a novel "Tricolumn" architecture with complexity scaling only quadratically with the voxel-grid size.

We demonstrate the efficacy of our model on the real-life StanfordORB benchmark \cite{kuang2023stanfordorb} where, given few input views, we achieve performance significantly superior to existing feedforward methods, and performance comparable to significantly slower scene optimization methods.
Furthermore, \themethod's environment map predictor is significantly superior to all existing methods achieving \TODO{XXX\%} better environment reconstruction error.


% \begin{figure}[t]
%  \centering
%  \includegraphics[width=\linewidth]{figs/0_Pulling.pdf}
%  \caption{
%      \textbf{PBR LRM.} 
%  }
%  % \vspace{-0.5cm}
%  \label{fig:pulling}
% \end{figure}

==> sec/3_method_old.tex <==
\section{Methodology [OLD]}
\label{sec:Methodology}

\begin{figure*}[t]
 \centering
 \includegraphics[width=\textwidth]{figs/1_Pipeline.pdf}
 \caption{
     \textbf{Proposed architecture.} Input views are processed together with their foreground masks and camera poses by a pretrained feature extractor. Resulting image and camera features are used by a Diffusion Transformer (DiT) model to predict a 3D volumetric representation of the scene, and a second DiT model to predict the scene's illumination. The 3D representation is then rendered to obtain the scene's material property, normal, and opacity images from the target points of view. Using these rendered images together with the predicted illumination we can obtain an approximate physically-shaded image of the scene.
 }
 % \vspace{-0.5cm}
 \label{fig:pipeline}
\end{figure*}

Our method aims to reconstruct real-life 3D objects along with their material properties from a small set of posed input views.
We achieve this by taking an LRM architecture and equipping it with an illumination prediction model and a differentiable physically-based rendering shader.
% By utilizing predicted material properties, illumination, and scene geometry, we are able to reconstruct shaded images.
In the following, we first cover an overview of LRMs and the physically-based rendering model we use.
Then, we detail the illumination estimation model as well as the .
We end with the losses used to supervise each component of the LRM.

\subsection{Preliminaries}
\mysection{Physically-Based Rendering}  
\label{sec:pbr_shader}
With knowledge of a scene's illumination, geometry, and materials properties it is possible to estimate the outgoing radiance at any point.
We do this by using the surface reflectance equation in \cref{eq:light_transport}.

\begin{equation}
    \mathbf{L}_o = \int\limits_\Omega (\mathbf{k}_d \frac{\mathbf{a}}{\pi} + \mathbf{f}_s) \mathbf{L}_i \langle \mathbf{\omega}_i,  \mathbf{n} \rangle d\mathbf{\omega}_i, \quad
    % \mathbf{L}_d = \mathbf{k}_d \frac{\mathbf{a}}{\pi} \int\limits_\Omega  \mathbf{L}_i \langle \mathbf{\omega}_i, \mathbf{n} \rangle d \mathbf{\omega}_i , \quad
    % \mathbf{L}_s = \int\limits_\Omega \mathbf{f}_s \mathbf{L}_i \langle \mathbf{\omega}_i, \mathbf{n} \rangle d\omega_i .
\label{eq:light_transport}
\end{equation}

\noindent where $\mathbf{L}_i$ is the incoming radiance, $\mathbf{a}$ is the object's diffuse albedo, and $\mathbf{k}_d$ and $\mathbf{f}_s$ are material properties dependent on the object's Bidirectional Reflectance Distribution Function (BRDF).
For clarity, we omit from notation the dependency of incoming radiance on $\mathbf{\omega}_i$ as well as the dependency of material properties on position $\mathbf{x}$.

Due to the complex integral involved, a multitude of approximations have been proposed in the field of computer graphics to efficiently estimate reflectance.
We rely on the split-sum approximation for image-based lighting, which relies on a representation of the scene's illumination as a spherical image which envelops the scene with an infinite radius.
Material properties are modeled by the Disney~\cite{karis2013real} microfacet BRDF parameterized by albedo, metalness, and roughness.

In order to apply this model to render a scene we require a representation of its geometry, a spherical image representing the scene's illumination, and estimates of objects' albedo, metalness, and roughness at surfaces.


\begin{figure}[t]
    \centering
    % \vspace{2.5cm}
    % \TODO{Jesus to export examples of envmaps + g.t. zeroverse renders}
    % \vspace{2.5cm}
    \includegraphics[width=\linewidth]{figs/2_zeroverse.pdf}
    \caption{
        \textbf{Examples from our PBR-env-zeroverse dataset.}
    }
    % \vspace{-0.5cm}
    \label{fig:zeroverse}
   \end{figure}
   


\mysection{Large Reconstruction Model}
The aim of the Large Reconstruction Model (LRM) is to obtain a 3D representation of a scene given a small set $\mathcal{I}$ of posed views of the scene.
First, an image feature extractor is used to obtain semantic features from the set of input views.
This feature extractor is composed of a pre-trained ViT which takes as input the set of colored images, foreground object masks and plucker embeddings to condition based on camera poses following~\cite{xu2023dmv3d}.
% We rely on a pre-trained ViT~\cite{vit} 
% Semantic features are extracted from the input views, which are then concatenated with plucker coordinates parameterizing the rays crossing each image pixel.
% The input views are processed by a diffusion transformer model and used to predict the 3D representation parameters.
% We parameterize the 3D scene with a tricolumn representation.
The extracted feature tokens are then processed by a diffusion transformer (DiT) to predict a 3D representation of the scene.
Using the memory efficient rendering proposed in lightplane~\cite{cao2024lightplane}, a target set of views is rendered from the 3D representation.
These views are then used to supervise the LRM via LPIPS and MSE losses.

\subsection{Tricolumn Representation}
A common 3D representation used in LRM models is the triplane representation~\cite{Chan2022eg3d} due to its simplicity and efficiency.
However, these benefits come at the cost of representation capacity.
We propose using a tricolumn representation instead.


\subsection{PBR LRM}
We aim at recovering material properties from the 3D representation in addition to the radiance.
This is achieved by extending the tricolumn representation to predict two additional channels representing the scene's metalness and roughness.
Similar to color images, it is straightforward to supervise the material property fields with ground truth renderings of material properties from synthetic datasets.

However, while color images can be readily obtained with commodity camera sensors, obtaining ground truth material properties is a costly endeavour.
Nonetheless, we aim to fine-tune our material supervision with real world data without access to ground truth material properties nor ground truth scene illumination.
% In this case the only supervision signal available is through shading
In this case the only supervision available is through the differentiable physically-based shader detailed in \cref{sec:pbr_shader}.
% However, in order to perform realistic shading we need an estimate of the scene's illumination.
% Realistic shading requires an estimate of the scene's illumination in addition to the material properties.
The shader requires modelling the scene's geometry, material properties, and illumination.
Both geometry and material properties are modelled with the tricolumn representation.

\subsection{Illumination Module}
In order to estimate the scene's illumination we propose using an additional DiT module.
% This is obtained by an additional diffusion transformer module which takes the input views and predicts a cubemap representation of the scene's lighting.
This additional DiT takes as input the feature tokens computed by the image feature extractor and predicts a cubemap representation of the scene's lighting.
% Equipped with material properties and a cubemap, we are able to efficiently estimate PBR shading via the splitsum approximation.
% The predicted shaded image is used to supervide the PBR model.


% There is an inherent ambiguity between the albedo and environment lighting.
Some information about a scene's illumination is captured in the background pixels of the input images.
We propose using this information as an additional supervisory signal to the scene illumination predictor.
% We supervise the cubemap predictions by using the input image's background in order to alleviate this issue.
The predicted cubemap is assumed to be surrounding the scene at infinity, and pixels falling outside of the object's foreground mask are assumed to hit the cubemap.
We calculate the intersection of each image ray with the cubemap in order to calculate a predicted background image.
This predicted background image is then composited with the foreground object prediction to obtain a composite scene image.
We supervise the composite image with LPIPS and MSE losses.


==> sec/method_separate_loss_section.tex <==
\section{Methodology}%
\label{sec:Methodology}

\input{figs/fig_zeroverse}
\input{figs/fig_pipeline}
\input{figs/fig_tricolumn}

\newcommand{\p}{\boldsymbol{p}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bomega}{\boldsymbol{\omega}}

We introduce \themethod, a model that can reconstruct the shape and material properties of real-life 3D objects from a small set of posed input views.
We obtain \themethod by equipping a LRM architecture with  predictors of the object's material properties and scene illumination and with a differentiable physically-based renderer.
In \cref{sec:preliminaries}, we start by reviewing the LRM and the PBR model we use.
Then, in \cref{sec:illumnation}, we  describe the predictors of the illumination and \dots
Finally, in \cref{XX}, we detail the learning formulation and the losses used to supervise each component of the LRM\@.

\subsection{Preliminaries}%
\label{sec:preliminaries}

\paragraph{Physically-Based Rendering.}%
\label{sec:pbr_shader}

In order to supervise our model utilizing the photometric loss, it is necessary to \emph{render} the reconstructed scene into an image, simulating the image formation process.
The color of each pixel is equal to the \emph{radiance}
$
\bL_o 
$
emitted by the imaged object point $\p\in\mathbb{R}^3$ in the direction of the camera.
With knowledge of a scene's illumination, geometry, and materials properties, it is possible to estimate the outgoing radiance at any such point according to the \emph{reflectance equation}:
%
\begin{equation}
\label{eq:reflectance}
\bL_o 
= 
\int\limits_\Omega 
\left(
    k_d 
    \frac{\mathbf{a}}{\pi} 
    +
    \mathbf{f}_s
\right)
\bL_i \,
\langle \bomega_i, \mathbf{n} \rangle \,
d\bomega_i.
\end{equation}
%
Here, $\bL_i$ is the incoming radiance, expressing the scene illumination falling at the imaged point $\p$.
The integral is carried over a half sphere $\Omega$ of incoming directions $\bomega_i$ determined by the surface normal $\mathbf{n}$.
The factor in parenthesis is a model of the the object's Bidirectional Reflectance Distribution Function (BRDF) which tells how the incoming radiance reflects off the object's surface into various directions.
The first term is the \emph{diffuse component}, and is parameterized by the object's diffuse albedo $\mathbf{a}$ and a constant $k_d$, both of which do not depend on direction;
in the integral, this term thus averages all incoming radiance over the hemisphere.
The second term $\mathbf{f}_s$ is the \emph{specular component} of the BRDF, which expresses any directional effect, such as reflections or highlights.
Note that $\bL_i$ is a function of the incoming direction $\bomega_i$ and the specular BRDF $\mathbf{f}_s$ is a function of both the incoming and the outgoing directions $\bomega_i$ and $\bomega_o$.
Radiances and BRDF depend on the light frequency too, of which we only model three RGB components.
Furthermore, all the quantities depend on the point position $\p \in \mathbb{R}^3$.
We omit these details for compactness.

Due to the complex integral in \cref{eq:reflectance}, a multitude of approximations have been proposed in computer graphics to efficiently estimate the reflectance equation~\eqref{eq:reflectance}.
We rely on the split-sum approximation for image-based lighting, which relies on a representation of the scene's illumination as a spherical image which envelops the scene with an infinite radius.\todo{Citation needed.}
The BRDF follows the Disney~\cite{karis2013real} microfacet BRDF model, and is parameterized by the albedo $\mathbf{a}$ and the metalness and roughness at each point.
We further assume that $\bL_i$ is constant in space (hence we do not account for shadows cast by the object itself).

In summary, in order to apply this model to render an image of the object, we require an estimate of the object 3D shape and of its albedo, metalness, and roughness at its surfaces.
We also require a spherical image representing the directional function $\bL_i$, known as an \emph{environment map}.

\paragraph{Large Reconstruction Model (LRM).}

The aim of LRM~\cite{hong24lrm:} is to map a small set of posed views $\mathcal{I}$ of the scene to a 3D reconstruction $V$.
LRM first extracts semantic features $y$ from the set of input views, utilizing a pre-trained DINO~\cite{oquab24dinov2:} Vision Transformer (ViT)~\cite{dosovitskiy21an-image}.
We further follow~\cite{xu24dmv3d:} and feed into the ViT encoder the RGB images, the masks of the foreground object to be reconstructed,  and the Pl{\"u}cker embeddings~\cite{sitzmann21light} to represent the cameras.

The extracted feature tokens are then used via cross-attention to condition the transformer architecture from Diffusion Transformer (DiT)~\cite{peebles23scalable} $\Phi$ which is tasked with predicting the 3D representation of the scene.
% \todo{Do we actually do diffusion here, or is this just the same architecture? The same architecture, with 16 layers. There are additional splatter layers added before layers 0, 8, and 15 for the tricolumn version.}
The tokens in this transformer encode the 3D representation of the scene, realizing a mapping $V = \Phi(V_0| y)$, where $V_0$ are the initial values of the tokens (learned and fixed).
A crucial design choice is how to construct the tokens $V$ manipulated by this transformer, which is discussed in \cref{sec:tricolumn}.

Finally, using the memory efficient rendering algorithm proposed in LightplaneLRM~\cite{cao2024lightplane}, a target set of views is rendered from the 3D representation.
These views are then used to supervise the LRM via the the training losses detailed in \cref{sec:losses}.
% \begin{equation}
% \mathcal{L} = \mathcal{L}_\text{MSE} + \mathcal{L}_\text{LPIPS} + \methcal{L}_\text{depth} + \mathcal{L}
% \end{equation}
% where LPIPS and MSE losses

\todo{We will have to write more explictly the learning formulation, and all the losses we use}

\subsection{Tricolumn representation}%
\label{sec:tricolumn}

\todo{AV\@: please check this description to ensure that it is correct, and perhaps provide some additional details on the recombination fucntion $f$.}

Crucial to the LRM design is the representation of the 3D scene, which is encoded as a set of volumetric functions expressing opacity and material properties at every point $\p \in \mathbb{R}^3$ in space.
A simple and effective option~\cite{sun22direct} to encode a volumetric function $V: \mathbb{R}^3 \rightarrow \mathbb{R}^C$ is to use a voxel grid $V \in \mathbb{R}^{C\times D \times H \times W}$.
Then, the value $V(\p) \in \mathbb{R}^C$ of the function is obtained by interpolating the voxel values at the nearest grid points.
To predict the voxel grid $V$ with the transformer of \cref{sec:preliminaries} we could, in principle, assign one token to each voxel.
However, the number $WHD$ of voxels grows cubically with the resolution of the grid, which makes this approach impractical.

The alternative adopted by models like~\cite{hong24lrm:,siddiqui24meta} is to use a \emph{triplane} representation~\cite{chan22efficient}.
In this case, the volumetric function is represented by three 2D grids 
$
V_{xy}\in \mathbb{R}^{K \times H \times W},
$
$
V_{yz}\in \mathbb{R}^{K \times W \times D},
$
and
$
V_{zx}\in \mathbb{R}^{K \times D \times H}.
$
The volumetric function at $\p=(x,y,z)$ is then expressed as
\begin{equation}\label{eq:triplane}
V(x,y,z) = f(
    V_{xy}(x, y),
    V_{yz}(y, z),
    V_{zx}(z, x)
),
\end{equation}
where $f : \mathbb{R}^{K \times K \times K} \rightarrow \mathbb{R}^C$ is a point-wise mixing function (e.g., a MLP applied to the concatenation of the three $K$-dimensional feature vectors).
Utilized in a transformer, this has the advantage of reducing the number of tokens to $WH + HD + DW$ only.
However, the disadvantage is that information is mixed between different voxels, which sometimes leads to artifacts.

We thus propose a novel \emph{tricolumn} representation instead.
This is similar to triplane as it uses a plane instead of a volume of tokens; however, each feature vector is in itself a column of corresponding voxel cells, so that voxel-specific information is represented directly.

In detail, we consider a plane of feature vectors $V_{xy}\in \mathbb{R}^{(CD)\times H\times W}$.
Because this is a plane, there are only $HW$ tokens, which are easily handled by the transformer.
However, $V_{xy}$ can be reshaped into a  $C \times D \times H \times W$ voxel grid by unfolding the first dimension.
We use the symbol $V_{xy}(x,y;z) \in \mathbb{R}^C$ to denote the feature vector obtained by interpolating this grid in 3D.

When three such planes are used, the full feature vector at $\p$ is decoded as:
\begin{equation}
\label{eq:tricolumn}
V(x,y,z)
=
f(
    V_{xy}(x,y;z),
    V_{yz}(y,z;x),
    V_{zx}(z,x;y)
).
\end{equation}
Note that this construction is strictly different from the triplane equation~\eqref{eq:triplane} as each term depends on all three spatial coordinates.

\subsection{PBR reconstruction model}%
\label{sec:pbr_lrm}

The LRM models of~\cite{hong24lrm:,xu24dmv3d:} only recover the shape and radiance of the scene.
Like in~\cite{siddiqui24meta}, we extend the LRM to also recover the material properties.
We do so by extending the tricolumn representation to predict albedo (instead of radiance), two additional channels representing the scene's metalness and roughness, and three additional channels representing the scene's normal vectors.

\paragraph{Learning formulation.}

Reconstruction models that predict radiance can be supervised by \emph{rendering} the predicted 3D scene into images and comparing these to training views, using a photometric loss.
In our case, however, the model does not predict radiance, but albedo, roughness, and metalness, which cannot be rendered into a `shaded' image unless illumination is also known.

A simple approach for supervising the model that does not require knowledge of illumination is to render albedo, roughness, and metalness directly as image channels, and compare these to the ground truth renders of the same.
However, this is only possible if the ground-truth material properties are available, which is not the case for real-world data, where only shaded images are available.



In order to fine-tune our model using real data, then, it is necessary to also estimate the scene illumination.
With this, we can then use the differentiable physically-based shader detailed in \cref{sec:pbr_shader} to render the shaded scene appearance, and compare that to the input images using the photometric loss.
We explain next (\cref{sec:illumnation}) how illumination is predicted.

% material supervision with real world data without access to ground truth material properties nor ground truth scene illumination.
% In this case, the only supervision available is through the differentiable physically-based shader detailed in \cref{sec:pbr_shader}.
% The shader requires modelling the scene's geometry, material properties, and illumination.
% Both geometry and material properties are modelled with the tricolumn representation.

% Similar to color images, it is straightforward to supervise the material property fields with ground truth renderings of material properties from synthetic datasets.

% However, while color images can be readily obtained with commodity camera sensors, obtaining ground truth material properties is a costly endeavour.
% Nonetheless, we aim to fine-tune our material supervision with real world data without access to ground truth material properties nor ground truth scene illumination.
% In this case, the only supervision available is through the differentiable physically-based shader detailed in \cref{sec:pbr_shader}.
% The shader requires modelling the scene's geometry, material properties, and illumination.
% Both geometry and material properties are modelled with the tricolumn representation.

\subsection{Illumination module}%
\label{sec:illumnation}

In order to estimate the scene's illumination we propose using an additional DiT module.
This additional DiT takes as input the feature tokens $y$ computed by the image feature extractor and predicts a cubemap representation of the scene's lighting.
Recall that a cubemap is a function $C \rightarrow \mathbb{R}^3$ that assigns every point $\p$ of the cube surface $C = \{ \| \p \|_\infty = 1\}$ to the radiance $\bL_i(\bomega_i)$ incoming from direction $\bomega_i \propto -\p$, and is thus a representation of the environment illumination (this works because we assume that the function $\bL_i$ only depends on direction, but not on position).
The cubemap is unfolded to a collection of six 2D images, which are then predicted by the DiT module.

\paragraph{Supervision.}

In synthetic data, the cubemap is known and its predictor can be supervised directly.
In real data, the cubemap is observed indirectly via the effect it has on the object appearance according to the reflectance equation~\eqref{eq:reflectance}, which provides only weak supervision.

We note, however, that the \emph{scene background} visible in the input images is, to a first approximation, equal to the function $\bL_i$, and can thus provide direct supervision of the latter.
We can \emph{render} the background observed from any given camera by assigning to each pixel the color
$
\bL_i(\bomega_i) = C(\bomega_i / \|\bomega_i\|_\infty)
$
of the incoming radiance from the direction $\bomega_i$ of the pixel's ray.
% Some information about a scene's illumination is captured in the background pixels of the input images.
% We propose using this information as an additional supervisory signal to the scene illumination predictor.
% The predicted cubemap is assumed to be surrounding the scene at infinity, and pixels falling outside of the object's foreground mask are assumed to hit the cubemap.
% We calculate the intersection of each image ray with the cubemap in order to calculate a predicted background image.
This predicted background image is then composited with the foreground object prediction to obtain a composite scene image.
We supervise the composite image with LPIPS and MSE losses.
\todo{This should be linked to the learning formulation section, so all losses are in one place. Do you have a separate loss for this, or is this just lumped together in the overall perceptual loss? It's all lumped together in the perceptual loss. The final losses for real data are LPIPs and MSE on the full img, mask BCE, depth L1, self-supervised normal cosine distance, and TV loss for albedo, depth, and normals. Synthetic data additionally has huber losses for albedo, metal, rough, gt normals, and envmap}

\subsection{Losses}%
\label{sec:losses}
As detailed in the precious sections, we take advantage of synthetic data for supervision when available, and get supervision for real data through our differentiable shader.
In the following, we detail the losses used when synthetic data is available followed by the losses calculated on all data.

\paragraph{Synthetic Data Only.}
Masked pixel-wise loss for albedo, metalness, roughness, normals, and latlong envmap images.
\begin{equation}\label{eq:synthetic_image}
\mathcal{L}_{S_\text{m}} = \text{huber}(\mathcal{M}(i)\mathcal{I}_{\text{m}}(i) - \mathcal{M}(i)\hat{\mathcal{I}}_{\text{m}}(i))
\end{equation}


\paragraph{Real and Synthetic Data.}
BCE loss on mask
\begin{equation}\label{eq:real_data_MSE}
\mathcal{L}_{M} = \text{BCE}(\mathcal{M}(i), \hat{\mathcal{M}(i)})
\end{equation}

LPIPS and MSE losses on full composite image
\begin{equation}\label{eq:all_data_photometric}
\mathcal{L}_{R} = \text{LPIPS}(\mathcal{I}(i), \hat{\mathcal{I}}(i)) + \|(\mathcal{I}(i) - \hat{\mathcal{I}}(i))\|^2
\end{equation}

L1 loss on masked depth image
\begin{equation}\label{eq:all_data_MSE}
\mathcal{L}_{d} = \|(\mathcal{M}(i)\mathcal{I}(i) - \mathcal{M}(i)\hat{\mathcal{I}}(i))\|
\end{equation}

Self-supervised:
Masked normals loss from pseudo-normals estimated from the gradient of opacity at surface points.
\begin{equation}\label{eq:all_data_normal_opacity}
\mathcal{L}_{N} = 1 - \langle \mathcal{M}(i) \bar{\mathcal{I}}_{\text{n}}(i),  \mathcal{M}(i) \hat{\mathcal{I}}_{\text{n}}(i) \rangle
\end{equation}
\begin{equation}\label{eq:pseudo_normal}
% \bar{\mathcal{I}}_{\text{n}}(i) = \nabla \sigma(\pi^{-1}(i, d(i)))
\bar{\mathcal{I}}_{\text{n}}(i) = \nabla \sigma(\pi^{-1}(i, d))
\end{equation}


TV regularization on albedo, depth, and normal images
\begin{equation}\label{eq:all_data_TV}
\mathcal{L}_{\text{TV}_\text{m}} = \text{TV}(\hat{\mathcal{I}}_{\text{m}}(i))\
\end{equation}









